Total Solar Eclipse White Light Images as a Benchmark for PFSS Coronal Magnetic Field Models: An In-Depth Analysis over a Solar Cycle

Potential Field Source Surface (PFSS) models are widely used to simulate coronal magnetic fields. PFSS models use the observed photospheric magnetic field as the inner boundary condition and assume a perfectly radial field beyond a ``Source Surface" ($R_{ss}$). At present, total solar eclipse (TSE) white light images are the only data that delineate the coronal magnetic field from the photosphere out to several solar radii ($R_\odot$). We utilize a complete solar cycle span of these images between 2008 and 2020 as a benchmark to assess the reliability of PFSS models. For a quantitative assessment, we apply a rolling Hough transform (RHT) to the eclipse data and corresponding PFFS models to measure the difference, $\Delta\theta$, between the data and model magnetic field lines throughout the corona. We find that the average $\Delta\theta$, $\langle\Delta\theta\rangle$, can be minimized for a given choice of $R_{ss}$ depending on the phase within a solar cycle. In particular, $R_{ss}\approx1.3 \ R_\odot$ is found to be optimal for solar maximum, while $R_{ss}\approx3 \ R_\odot$ yields a better match at solar minimum. However, large ($\langle\Delta\theta\rangle>10^\circ$) discrepancies between TSE data and PFSS-generated coronal field lines remain regardless of the choice of source surface. Yet, implementation of solar cycle dependent $R_{ss}$ optimal values do yield more reliable PFSS-generated coronal field lines for use in models and for tracing in-situ measurements back to their sources at the Sun.

==> packages.tex <==

%% if you use PostScript figures in your article
%% use the graphics package for simple commands
%% \usepackage{graphics}
%% or use the graphicx package for more complicated commands
%% \usepackage{graphicx}
%% or use the epsfig package if you prefer to use the old commands
%% \usepackage{epsfig}

%% The amssymb package provides various useful mathematical symbols
\usepackage{amssymb}
%% The amsthm package provides extended theorem environments
%% \usepackage{amsthm}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{aas_macros}
\usepackage{rotating}
\usepackage{url}
\usepackage{morefloats} 
\usepackage{float}
\usepackage{threeparttable}
\usepackage{rotating}
\usepackage{longtable}
\usepackage{array}
\usepackage{color}
%Image-related packages
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage[utf8]{inputenc}
\usepackage[export]{adjustbox}
\usepackage{wrapfig}
\usepackage{lineno}
\usepackage[table]{xcolor}
%\usepackage{subcaption}
%\usepackage[caption = false]{subfig}                 % necessary???
%\usepackage[hmargin=1.5cm,vmargin=1.5cm]{geometry}   % necessary???

